MEDIRL: Predicting the Visual Attention of Drivers via Maximum Entropy Deep Inverse Reinforcement Learning

Inspired by human visual attention, we propose a novel inverse reinforcement learning formulation using Maximum Entropy Deep Inverse Reinforcement Learning (MEDIRL) for predicting the visual attention of drivers in accident-prone situations. MEDIRL predicts fixation locations that lead to maximal rewards by learning a task-sensitive reward function from eye fixation patterns recorded from attentive drivers. Additionally, we introduce EyeCar, a new driver attention dataset in accident-prone situations. We conduct comprehensive experiments to evaluate our proposed model on three common benchmarks: (DR(eye)VE, BDD-A, DADA-2000), and our EyeCar dataset. Results indicate that MEDIRL outperforms existing models for predicting attention and achieves state-of-the-art performance. We present extensive ablation studies to provide more insights into different features of our proposed model.

==> tables/driving-decision.tex <==
\begin{table}[htbp]
\centering
\small
\scalebox{0.85}{% 
\begin{tabular}{c c}
\toprule
\textbf{driving-task} & \textbf{driving-intention} \\
\hline
\hline
Merging-in & {front, back}\\
\hline
lane-keeping & yield, pass\\
\hline
braking & {stop}\\
\bottomrule
\end{tabular}}
\vspace{.3em}
\caption{Driving tasks and intentions.\label{tbl:driving-decision}}
\end{table} 



% \newlength{\oldintextsep}
% \setlength{\oldintextsep}{\intextsep}
% \setlength\intextsep{0pt}
% \begin{wraptable}{r}{4.2cm}
% \small
% \centering
% \label{tbl:driving-decision}
%  \scalebox{0.85}{
% \begin{tabular}{c c c}
% \toprule
% \textbf{driving-task} & \textbf{driving-intention} \\
% \hline
% Merging-in & {front, back}\\
% \hline
% lane-keeping & yield, pass\\
% \hline
% braking & {stop}\\
% \hline
% \end{tabular}}
% \caption{\scriptsize{Driving tasks and intentions}}
% \end{wraptable} 
% \vspace{-1.5mm}

==> tables/features-types.tex <==
\setlength{\abovecaptionskip}{-0.5pt}
\setlength{\belowcaptionskip}{-2pt}
\setlength\intextsep{1pt}
\begin{table*}[htbp]
\centering 
\small\addtolength{\tabcolsep}{-2pt}
    \scalebox{0.9}{%(E_{\text{dens}}, E_{\text{semantic}}, E_{\text{illum}})
    \begin{tabular}{l| c c c c}
      \toprule % <-- Toprule here
      \textbf{Data Source} & \textbf{Feature} & \textbf{Type} & \textbf{Values} & \textbf{Scale}\\
      \hline
      \hline
      \multirow{3}{*}{eye movement~($f_M$)} & location & integer & (0-6400) & per fixation in a frame\\
      & distance & categorical & near-reach, medium-reach, far-reach &per fixation in a frame\\ 
      & fixation & integer & [110ms-447ms] & per fixation in a frame\\
       & light & integer & 0/1 & per fixation in a frame\\
      \hline
      \multirow{2}{*}{driving environment~($f_E$)} & density & proportion & [0\%-58\%] & per frame\\
      & semantic & categorical & \textcolor{red}{categories$_{\text{list}}$ }& per frame\\
      & illumination & categorical & 0/1 & per frame\\
      \hline
      vehicle information~($f_V$) & speed & categorical & slow, normal, fast & per frame\\
     \bottomrule % <-- Bottomrule here
    \end{tabular}}
    \caption{Saliency-specific feature vectors from the VFE module.\label{tbl:state-feature}}
\end{table*}


% \end{small}
%\textcolor{red}{113, 299, 350, 845, ....}




==> tables/results.tex <==
\begin{table*}[t!]
\centering
\small\addtolength{\tabcolsep}{-.2pt}

\scalebox{0.58}{

\begin{tabular}{lr}
{
\begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|}
\toprule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Data}}}&\multirow{2}{*}{\diagbox{Method}{Task}} &\multicolumn{3}{c|}{Merging-in} & \multicolumn{3}{|c|}{Lane-keeping}& \multicolumn{3}{|c|}{Braking}\\
\cline{3-11}
           &    &   CC\uparrow  &   s-AUC\uparrow & KLD\downarrow  & CC\uparrow    &   s-AUC\uparrow & KLD\downarrow  &   CC\uparrow  &s-AUC\uparrow & KLD\downarrow\\\hline
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\scriptsize{DR(eye)VE~\cite{palazzi2018predicting}}}}}&
Multi-branch~\cite{palazzi2018predicting} & 0.48 & 0.41  & 2.80 & 0.55 & 0.51 & 1.87 & 0.71 & 0.53 & 2.20 \\
&HWS~\cite{xia2018predicting}          & 0.51 & 0.48  & 2.12 & 0.75 & 0.49 & 1.72 & 0.74 & 0.57 & 1.99 \\
&SAM-ResNet~\cite{cornia2018predicting}    & \textbf{0.78} & 0.54  & 2.01 & 0.80 & 0.59 & 1.80 & 0.79 & 0.69 & 1.89 \\
&SAM-VGG~\cite{cornia2018predicting}      & \textbf{0.78} & 0.55  & 2.05 & 0.82 & 0.56 & 1.84 & 0.80 & 0.66 & 1.81 \\
&TASED-NET~\cite{min2019tased}      & 0.68 & 0.59  & 1.89 & 0.73 & 0.61  & 1.71 & 0.70 & 0.62  & 1.89 \\
&\textit{GT}              &  \textit{1}   &\textit{ 0.95}  & \textit{0.01} & \textit{1}   &\textit{ 0.98} & \textit{0}   & \textit{1}  & \textit{0.99} & \textit{0}   \\
&\textbf{MEDIRL} & \textbf{0.78} & \textbf{0.69}  &\textbf{ 0.88} & \textbf{0.89} & \textbf{0.67} & \textbf{0.75} & \textbf{0.85} &\textbf{ 0.63} & \textbf{0.82} \\ \hline \cline{2-11}
%------------------
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\scriptsize{BDD-A~\cite{yu2020bdd100k}}}}}&
Multi-branch~\cite{palazzi2018predicting} & 0.58 & 0.51  & 2.08 & 0.75 & 0.72 & 2.0  & 0.69 & 0.77 & 2.04 \\
&HWS~\cite{xia2018predicting}          & 0.53 & 0.59  & 1.95 & 0.67 & 0.89 & 1.52 & 0.69 & 0.81 & 1.59 \\
&SAM-ResNet~\cite{cornia2018predicting}   & 0.74 & 0.61  & 2.00 & 0.89 & 0.79 & 1.83 & 0.85 & 0.88 & 1.89 \\
&SAM-VGG~\cite{cornia2018predicting}      & 0.76 & 0.62  & 1.79 & 0.89 & 0.82 & 1.64 & 0.86 & 0.87 & 1.85 \\
&TASED-NET~\cite{min2019tased}      & 0.73 & 0.68  & 1.83 & 0.81 & 0.66  & 1.17 & 0.87 & 0.88  & 1.12 \\
&\textit{GT}              &  \textit{1}   & \textit{0.97}  & \textit{0.01} & \textit{1}   &\textit{ 0.99} & \textit{0}   & \textit{1 }  & \textit{0.98} & \textit{0}   \\
&\textbf{MEDIRL} & \textbf{0.82} &\textbf{ 0.79}  & \textbf{0.91} & \textbf{0.94} & \textbf{0.91} & \textbf{0.85} & \textbf{0.93} & \textbf{0.92} & \textbf{0.89 }\\ \hline \cline{2-11}
%-------------------
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\scriptsize{DADA-2000~\cite{fang2019dada}}}}}&
Multi-branch~\cite{palazzi2018predicting} & 0.44 & 0.53  & 3.65 & 0.69 & 0.54 & 2.85 & 0.67 & 0.64 & 2.91 \\
&HWS~\cite{xia2018predicting}        & 0.49 & 0.59  & 3.02 & 0.72 & 0.53 & 2.65 & 0.69 & 0.77 & 2.80 \\
&SAM-ResNet~\cite{cornia2018predicting}   & 0.65 & 0.61  & 2.39 & 0.78 & 0.64 & 2.32 & 0.75 & 0.81 & 2.34 \\
&SAM-VGG~\cite{cornia2018predicting}    & 0.68 & 0.60  & 2.41 & 0.76 & 0.62 & 2.24 & 0.75 & 0.80 & 2.35 \\
&TASED-NET~\cite{min2019tased}      & 0.69 & 0.66  & 1.98 & 0.78 & 0.69  & 1.87 & 0.80 & 0.81  & 1.45 \\
&\textit{GT}              & \textit{1}   & \textit{0.94}  & \textit{0.02} & \textit{1}   & \textit{0.98} & \textit{0}   & \textit{1}   & \textit{0.99} &\textit{0}   \\
&\textbf{MEDIRL} &\textbf{ 0.70} & \textbf{0.68}  & \textbf{1.31} & \textbf{0.89} & \textbf{0.71} & \textbf{0.92} & \textbf{0.81} & \textbf{0.88} &\textbf{ 0.99} \\ 
\bottomrule
\end{tabular}}
&
{
\begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|}
\toprule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Data}}}&\multirow{2}{*}{\diagbox{Method}{Task}} &\multicolumn{3}{c|}{Merging-in} & \multicolumn{3}{|c|}{Lane-keeping}& \multicolumn{3}{|c|}{Braking}\\
\cline{3-11}
           &    &   CC\uparrow  &   s-AUC\uparrow & KLD\downarrow  & CC\uparrow    &   s-AUC\uparrow & KLD\downarrow  &   CC\uparrow  &s-AUC\uparrow & KLD\downarrow\\\hline
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{DR(eye)VE~\cite{palazzi2018predicting}}}}&Multi-branch~\cite{palazzi2018predicting} &   0.36      &   0.37     &   6.46    &   0.51 & 0.49 & 4.80 & 0.69 & 0.49 &   3.38 \\
&HWS~\cite{xia2018predicting}     &   0.38      &   0.34   &   4.38    &   0.71 & 0.51 & 4.44 & 0.72 & 0.61 &   3.30 \\
&SAM-ResNet~\cite{cornia2018predicting}   &   0.49    &   0.48   &   4.29   &   0.73 & 0.55 & 3.90  & 0.74 & 0.66 &   3.27 \\
&SAM-VGG~\cite{cornia2018predicting}   &   0.50   &   0.47     &   4.31    &  0.74 & 0.53 & 3.95 & 0.75 & 0.64 &   3.29 \\
&TASED-NET~\cite{min2019tased}      & 04.8 & 0.46  & 3.95 & 0.74 & 0.55  & 3.81 & 0.76 & 65  & 3.23 \\
&\textbf{MEDIRL}   &  \textbf{ 0.51 } &  \textbf{ 0.51 }   &   \textbf{2.32}    &   \textbf{0.76} & \textbf{0.57} & \textbf{3.11} & \textbf{0.79} & \textbf{0.69} &   \textbf{3.07} \\ \hline 
%------------------
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{BDD-A~\cite{yu2020bdd100k}}}}&Multi-branch\cite{palazzi2018predicting} &   0.46      &   0.48 &   4.42   & 0.51 &0.61 & 3.57 & 0.61 & 0.64 &   3.08 \\
&HWS\cite{xia2018predicting}      &   0.41      &   0.47   &   4.36    &  0.69 & 0.81 & 3.55 & 0.67 & 0.68 &   2.86 \\
&SAM-ResNet~\cite{cornia2018predicting}   &   0.55     &   0.48  &   3.85    &  0.85 & 0.72 & 3.29  & 0.79 & 0.74 &   2.46 \\
&SAM-VGG~\cite{cornia2018predicting}   &   0.53      &   \textbf{0.49} &   3.92    & 0.84  &0.70 &  3.22 & 0.77 & 0.70  &   2.49 \\
&TASED-NET~\cite{min2019tased}      & 0.55 & \textbf{0.49}  & 3.78 & 0.84 & 0.71  & 3.12 & 0.77 & 0.76  & 2.47 \\
&\textbf{MEDIRL}   &   \textbf{0.58 } &   \textbf{0.49}    &   \textbf{2.81}    & \textbf{0.86}  &   \textbf{0.73}& \textbf{2.43} & \textbf{0.79} & \textbf{0.81} &   \textbf{2.30} \\ \hline
%-------------------
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{DADA-2000~\cite{fang2019dada}}}}&Multi-branch\cite{palazzi2018predicting} &   0.21      &   0.38 &   6.46    &   0.45 & 0.44 & 4.67 & 0.54 & 0.59 &   3.12 \\
&HWS\cite{xia2018predicting}     &   0.31      &   0.35   &   6.12    &   0.51 & 0.47 & 4.54 & 0.67 & 0.71 &   3.10 \\
&SAM-ResNet~\cite{cornia2018predicting}   &   0.33     &   0.38   &   5.28  & 0.65  &   0.56  & 4.42 & 0.77& 0.71  &   3.07 \\
&SAM-VGG~\cite{cornia2018predicting}   &   0.30      &   0.39    &   5.35    &  0.69 & 0.57 & 4.31 & 0.74& 0.69  &   3.10 \\
&TASED-NET~\cite{min2019tased}      & 0.32 & 0.38  & 4.76 & 0.68 & 0.57  & 3.99 & 0.73 & 0.74  & 3.01 \\
&\textbf{MEDIRL}   &  \textbf{ 0.41}  &   \textbf{0.45}    &   \textbf{3.79}  &  \textbf{0.73} & \textbf{0.60} & \textbf{2.51} & \textbf{0.75} & \textbf{0.79} &   \textbf{2.51} \\
\bottomrule
\end{tabular}}
\end{tabular}

}
\vspace{.3em}
\caption{Evaluation results for the task specific visual attention allocation tested on benchmarks (left) and on EyeCar (right).\label{tbl:results}}
\end{table*}



